TRAPP: An Efficient Point-to-Point Path Planning Algorithm for Road Networks with Restrictions

Path planning is a fundamental problem in road networks, with the goal of finding a path that optimizes objectives such as shortest distance or minimal travel time. Existing methods typically use graph indexing to ensure the efficiency of path planning. However, in real-world road networks, road segments may impose restrictions in terms of height, width, and weight. Most existing works ignore these road restrictions when building indices, which results in returning infeasible paths for vehicles. To address this, a naive approach is to build separate indices for each combination of different types of restrictions. However, this approach leads to a substantial number of indices, as the number of combinations grows explosively with the increase in different restrictions on road segments. In this paper, we propose a novel path planning method, TRAPP(Traffic Restrictions Adaptive Path Planning algorithm), which utilizes traffic flow data from the road network to filter out rarely used road restriction combinations, retain frequently used road restriction combinations, and build indices for them. Additionally, we introduce two optimizations aimed at reducing redundant path information storage within the indices and enhancing the speed of index matching. Our experimental results on real-world road networks demonstrate that TRAPP can effectively reduce the computational and memory overhead associated with building indices while ensuring the efficiency of path planning.

==> paper-sketch.tex <==
intro介绍几本问题（把问题说清楚），并给出解决方案（intuition）
preliminary，介绍basic definition formally和sota的方法框架，road network with restrictions，vehicle（因为要说车辆的性质），Feasible path（相对于车辆来说的可行路径），shortest feasible path，然后说出我们的path plan的目的是找出shortest feasible path对于给定的vehicle。接下来说shortcut，简单解释为啥要shortcut（为了加速online path planning）。但是在限制情况传统的不考虑限制，在shortuct帮助下找到的最短路径可能不行。因此考虑限制的情况下，我们应该针对不同的限制记录不同的路径，在定义这个之前，我们先提供exit/entry vertex，shortcut path，feasible shorcut path，shortest feasible shortcut path。（exit/entry是为了便于后边的shortcut path的介绍，因为shortcut path要限制在子图内）。介绍完这些后，在说shortcut，就是包含很多shortest feasible shortcut path针对不同的restirciton combinations。

problem statement（第三章）说下2阶段框架，介绍的过程中强调shortcut很重要，极大加速了online查找过程。然后再说，当有限制的时候，正如我们在第二章介绍了，shortcut应该存多个路径针对不同的限制。这样我们在查找的时候，根据车的属性，查找可通过的限制，即可得到对应的路径。从而可以返回path plan的结果。然而在实际的路网中每个限制可能有多个值，多个限制的组合是一种爆炸的结果。如图XX所示，所有的组合有120种。首先为每一种组合构件并存储，需要大量的预处理时间和大量的存储空间。其次，当组合非常多的时候，在线查找的过程需要匹配合适的限制，这导致匹配过程非常长，甚至超过查找过程。然后formal地引出our goal。

%前面应该有一个定理，说明越宽泛，即被支配（组合之间的支配，vehicle之间的支配），vehicle被支配，则被支配的车可以在支配的车的feasible path上走，同样，组合之间的支配，支配的比被支配的要大于等于。

还应该说一下限制下的路径选择，怎么选，在shortcut的情况下，这些都没说其实。

